Zero-Resource Multi-Dialectal Arabic Natural Language Understanding

A reasonable amount of annotated data is required for fine-tuning pre-trained language models (PLM) on downstream tasks. However, obtaining labeled examples for different language varieties can be costly. In this paper, we investigate the zero-shot performance on Dialectal Arabic (DA) when fine-tuning a PLM on modern standard Arabic (MSA) data only -- identifying a significant performance drop when evaluating such models on DA. To remedy such performance drop, we propose self-training with unlabeled DA data and apply it in the context of named entity recognition (NER), part-of-speech (POS) tagging, and sarcasm detection (SRD) on several DA varieties. Our results demonstrate the effectiveness of self-training with unlabeled DA data: improving zero-shot MSA-to-DA transfer by as large as $\sim$10\% F$_1$ (NER), 2\% accuracy (POS tagging), and 4.5\% F$_1$ (SRD). We conduct an ablation experiment and show that the performance boost observed directly results from the unlabeled DA examples used for self-training. Our work opens up opportunities for leveraging the relatively abundant labeled MSA datasets to develop DA models for zero and low-resource dialects. We also report new state-of-the-art performance on all three tasks and open-source our fine-tuned models for the research community.

==> misc.tex <==


\begin{table*}[h]
\begin{center}
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule

\textbf{Model}
& 
    & \multicolumn{3}{c|}{\textbf{Common Tags}}
        &  \multicolumn{3}{c}{\textbf{All Tags}} \\

\hline
& \textbf{MSA} & \textbf{EGY} & \textbf{GLF} & \textbf{LEV}  & \textbf{EGY} & \textbf{GLF} & \textbf{LEV} \\
\hline
XLM-R\textsubscript{BASE} & 96.3 & 82.79 & 83.97 & 80.25 & & & \\ 
\hline
XLM-R\textsubscript{BASE}, ST, $S=50$ & - & 84.08 & \textbf{85.38} & \textbf{82.05} &&&  \\
XLM-R\textsubscript{BASE}, ST, $S=100$ & - & \textbf{84.17} & 84.99 & 81.27 &&& \\
XLM-R\textsubscript{BASE}, ST, $S=200$ & - & 82.41 & 84.45 & 81.51  &&&\\ 
\hline
XLM-R\textsubscript{BASE}, ST, $\tau=0.90$ & - & 83.22 & 84.21 &  81.32&&& \\ 
XLM-R\textsubscript{BASE}, ST, $\tau=0.85$& - & 83.65 & 83.77 &  81.17 &&&  \\ 
XLM-R\textsubscript{BASE}, ST, $\tau=0.80$ & - & 80.59 & 83.97 &  80.59 &&& \\ 


\hline

\end{tabular}
\end{center}
\caption{\label{Tab:zero-all} Zero-shot transfer results on DA For NER (Macro F$_1$) and POS Tagging (Accuracy). Models are trained on MSA only and evaluated on DA.}
\end{table*}



%%%%%%%%%
AQC for journal


\begin{table*}[h]
\begin{center}
\begin{tabular}{llllll}
\toprule
\bf Model &  \bf AQC  &  \bf MSA & \bf EGY & \bf GULF & \bf LEV  \\ \hline
CRF \cite{darwish2018multi}   & ~ ~ -- &  93.6  & 92.9 & 87.8 & 87.9 \\
WC-BiLSTM  (ours) & 91.65   & 94.63  & 93.41 & 88.79 & 86.13\\
mBERT (ours) & 94.83 & 90.57  &  92.88  & 87.85 & 72.30  \\

XLM-R\textsubscript{BASE} (ours) & \textbf{96.70} & 96.30 & 94.70 & 92.18 & 89.98\\
XLM-R\textsubscript{LARGE} (ours)  & 96.59 & \bf 98.21 & \bf 97.00 & \bf 94.41 & \bf 93.19\\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{Tab:pos} Test set accuracy for POS Tagging.}
\end{table*}

%%%%%%%%%%%%



\begin{figure}[t] 
\hspace{4cm}
\includegraphics[width=7cm, height=3cm]{self-training-confusion-mat.pdf}
\caption{Comparison of fine-tuned model (FT) prediction categories (left) and the fine-tuned+self-trained model (ST) prediction categories (right). \note[mam]{I was expecting this to be a confusion matrix of the actual tags (loc, per, org). Unless we add a table of these tags, I think we should just remove this one as its info. is already in the other table.}}
\label{fig:ft-st-comp}
\end{figure}

%%%%%%%%%%%%
\begin{table}[h]
    \centering

    \begin{tabular}{c|c|c|c}
        \toprule
        \textbf{Measure}  &  \textbf{FT} & \textbf{ST} & \textbf{\% improvement} \\
        \hline
        True Positives & 159 & 159 & 0 \% \\
        False Positive & 359 & 264 & \textbf{26.5 \%}\\
        False Negative & 162 &168 & -3.7 \% \\
        True Negative & 5,940 & 6,035 & 1.5 \% \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of error categories in percentage between the fine-tuned model (FT) and the model combining fine-tuned+self-trained (ST) model, based on the dialectal part of the dev set of the NER task. }
    \label{tab:st-fp}
\end{table}



\begin{table*}[h]
\begin{center}
%\footnotesize
\begin{tabular}{c|c|c|c|c}
\toprule

\textbf{Model}
   & \multicolumn{2}{c|}{\textbf{MSA}}
        &  \multicolumn{2}{c}{\textbf{DA}} 
        \\

\hline
 & \textbf{DEV} & \textbf{TEST} & \textbf{DEV} &  \textbf{TEST}\\
 \hline

XLM-R\textsubscript{BASE} & 65.64  & 68.68 &  61.66 & 60.17  \\
XLM-R\textsubscript{LARGE} & 67.81  & 71.55 &  62.28 & 62.90  \\



\bottomrule
\end{tabular}
\end{center}
\caption{\label{Tab:zero-all} Sarcasm Detection macro F1 on both MSA and DA subsets of Ar-Sarcasm when training on MSA only}
\end{table*}
